Minimal covers in the Weihrauch degrees

In this paper, we study the existence of minimal covers and strong minimal covers in the Weihrauch degrees. We characterize when a problem $f$ is a minimal cover or strong minimal cover of a problem $h$. We show that strong minimal covers only exist in the cone below $\mathsf{id}$ and that the Weihrauch lattice above $\mathsf{id}$ is dense. From this, we conclude that the degree of $\mathsf{id}$ is first-order definable in the Weihrauch degrees and that the first-order theory of the Weihrauch degrees is computably isomorphic to third-order arithmetic.

==> symbols.tex <==
\usepackage{ifthen}
\usepackage{xargs}

\usepackage{xcolor}

\usepackage{todonotes}
\setuptodonotes{inline}
\makeatletter


\newcommand{\textdef}[1]{\emph{#1}}

\newcommand{\st}{{}\,:\,{}}

\def\function{\@ifstar\@function\@@function}
\newcommand{\@function}[2]{#1 \to #2}
\newcommand{\@@function}[2]{\colon #1 \to #2}

\def\mfunction{\@ifstar\@mfunction\@@mfunction}
\newcommand{\@mfunction}[2]{#1 \rightrightarrows #2}
\newcommand{\@@mfunction}[2]{\colon #1 \rightrightarrows #2}

%\newcommand{\restrict}[1]{\ensuremath{\left. \hspace{-1mm} \right|_{#1}}}
\newcommand{\restrict}[1]{_{#1}}

\newcommand{\pfunction}[2]{:\subseteq #1 \to #2}
\newcommand{\pmfunction}[2]{:\subseteq #1 \rightrightarrows #2}

\newcommand{\dom}{\operatorname{dom}}
\newcommand{\id}{\operatorname{id}}

\newcommand{\Baire}{\mathbb{N}^\mathbb{N}}

\newcommand{\turingreducible}{\le_\mathrm{T}}
\newcommand{\turingabove}{\ge_\mathrm{T}}
\newcommand{\strictlyturingabove}{>_\mathrm{T}}
\newcommand{\turingequiv}{\equiv_\mathrm{T}}
\newcommand{\strictlyturingreducible}{<_\mathrm{T}}
\newcommand{\turingincomparable}{\,|_\mathrm{T}\,}

\newcommand{\medvedevreducible}{\le_\mathrm{M}}
\newcommand{\strictlymedvedevreducible}{<_\mathrm{M}}
\newcommand{\medvedevequiv}{\equiv_\mathrm{M}}
\newcommand{\geqM}{\geq_{\mathrm{M}}}
\newcommand{\medvedevincomparable}{~|_{\mathrm{M}~}}
\newcommand{\medvedevdegrees}{\mathcal{M}}
\newcommand{\medvedevsucc}[1]{\{ #1\}^+}
\newcommand{\NREC}{\mathrm{NR}}

\newcommand{\weireducible}{\le_{\mathrm{W}}}
\newcommand{\strictlyweireducible}{<_\mathrm{W}}
\newcommand{\weiequiv}{\equiv_{\mathrm{W}}}
\newcommand{\weiincomparable}{~|_{\mathrm{W}~}}
\newcommand{\weidegrees}{\mathcal{W}}

\newcommand{\str}[1]{({#1})}

\newcommand{\pairing}[1]{\langle #1 \rangle}
\newcommand{\concat}{\smash{\raisebox{.9ex}{\ensuremath\smallfrown} }}

\newcommand*{\theory}{\mathrm{Th}}

\newcommand{\question}[1]{{\color{red} #1}}
\newcommand{\warning}[1]{{\color{orange} #1}}



\makeatother

==> thref.tex <==
\makeatletter
\def\ifenv#1{
	\def\@tempa{#1}%
	\ifx\@tempa\@currenvir
	   \expandafter\@firstoftwo
	 \else
	   \expandafter\@secondoftwo
	\fi
}


\newcommand{\thlabel}[1]{%
	\label{#1}
	\begingroup
	\ifenv{theorem}{
		\def\@currentlabel{Theorem \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{unprovedtheorem}{
		\def\@currentlabel{Theorem \ref{#1}}
		\label{#1-th}
	}
 	{\ifenv{proposition}{
		\def\@currentlabel{Proposition \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{unprovedproposition}{
		\def\@currentlabel{Proposition \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{lemma}{
		\def\@currentlabel{Lemma \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{corollary}{
		\def\@currentlabel{Corollary \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{fact}{
		\def\@currentlabel{Fact \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{remark}{
		\def\@currentlabel{Remark \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{definition}{
		\def\@currentlabel{Definition \ref{#1}}
		\label{#1-th}
	}
	{\GenericWarning{No Environment Found}}}}}}}}}}
	\endgroup
}

\newcommand{\thref}[1]{\ref{#1-th}}

\makeatother
 
